Grover's Quantum Search Algorithm of Causal Multiloop Feynman Integrals

A proof-of-concept application of a quantum algorithm to multiloop Feynman integrals in the Loop-Tree Duality (LTD) framework is applied to a representative four-loop topology. Bootstrapping causality in the LTD formalism, is a suitable problem to address with quantum computers given the straightforward possibility to encode the two on-shell states of a propagator on the two states of a qubit. A modification of Grover's quantum search algorithm is developed and the quantum algorithm is successfully implemented on IBM Quantum and QUTE simulators.

==> PoS - Grovers quantum search algorithm of causal multiloop Feynman integrals/latexmkrc <==
###################################
#   Configuration script for build latex

#   The next lines are the original ones from source
#
#$pdf_previewer='zathura';
#$pdflatex='xelatex -synctex=1 %0 %S'
#@generated_exts=(@generated_exts, 'synctex.gz');

#   Compilation with Xelatex
$latex = 'latex --enable-write18 %O %S';
#$pdflatex='pdflatex -synctex=1 %0 %S';
#$pdf_mode=1;
$pdf_mode=5;
$dvi_mode=$postscript_mode=0;
#$dvipdf = "dvipdfm %O -o %D %S";


#   axodraw automation
add_cus_dep( "ax1", "ax2", 0, "axohelp");
sub axohelp {return system "axohelp \"$_[0]\"";}
$clean_ext .=" %R.ax1 %R.ax2;"

==> PoS - Grovers quantum search algorithm of causal multiloop Feynman integrals/main-references.tex <==
%\cite{Catani:2008xa}
\bibitem{Catani:2008xa}
S.~Catani, T.~Gleisberg, F.~Krauss, G.~Rodrigo and J.~C.~Winter,
%``From loops to trees by-passing Feynman's theorem,''
JHEP \textbf{09} (2008), 065
doi:10.1088/1126-6708/2008/09/065
[arXiv:0804.3170 [hep-ph]].
%150 citations counted in INSPIRE as of 18 Nov 2022

%\cite{Tomboulis:2017rvd}
\bibitem{Tomboulis:2017rvd}
E.~T.~Tomboulis,
%``Causality and Unitarity via the Tree-Loop Duality Relation,''
JHEP \textbf{05} (2017), 148
doi:10.1007/JHEP05(2017)148
[arXiv:1701.07052 [hep-th]].
%37 citations counted in INSPIRE as of 18 Nov 2022

%\cite{deJesusAguilera-Verdugo:2021mvg}
\bibitem{deJesusAguilera-Verdugo:2021mvg}
J.~de Jes\'us Aguilera-Verdugo, F.~Driencourt-Mangin, R.~J.~Hern\'andez-Pinto, J.~Plenter, R.~M.~Prisco, N.~S.~Ram\'\i{}rez-Uribe, A.~E.~Renter\'\i{}a-Olivo, G.~Rodrigo, G.~Sborlini and W.~J.~Torres Bobadilla, \textit{et al.}
%``A Stroll through the Loop-Tree Duality,''
Symmetry \textbf{13} (2021) no.6, 1029
doi:10.3390/sym13061029
[arXiv:2104.14621 [hep-ph]].
%16 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Ramirez-Uribe:2021ubp}
\bibitem{Ramirez-Uribe:2021ubp}
S.~Ram\'\i{}rez-Uribe, A.~E.~Renter\'\i{}a-Olivo, G.~Rodrigo, G.~F.~R.~Sborlini and L.~Vale Silva,
%``Quantum algorithm for Feynman loop integrals,''
JHEP \textbf{05} (2022), 100
doi:10.1007/JHEP05(2022)100
[arXiv:2105.08703 [hep-ph]].
%19 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Clemente:2022nll}
\bibitem{Clemente:2022nll}
G.~Clemente, A.~Crippa, K.~Jansen, S.~Ram\'\i{}rez-Uribe, A.~E.~Renter\'\i{}a-Olivo, G.~Rodrigo, G.~F.~R.~Sborlini and L.~Vale Silva,
%``Variational quantum eigensolver for causal loop Feynman diagrams and acyclic directed graphs,''
[arXiv:2210.13240 [hep-ph]].
%1 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Aguilera-Verdugo:2020set}
\bibitem{Aguilera-Verdugo:2020set}
J.~J.~Aguilera-Verdugo, F.~Driencourt-Mangin, R.~J.~Hern\'andez-Pinto, J.~Plenter, S.~Ramirez-Uribe, A.~E.~Renteria Olivo, G.~Rodrigo, G.~F.~R.~Sborlini, W.~J.~Torres Bobadilla and S.~Tracz,
%``Open Loop Amplitudes and Causality to All Orders and Powers from the Loop-Tree Duality,''
Phys. Rev. Lett. \textbf{124} (2020) no.21, 211602
doi:10.1103/PhysRevLett.124.211602
[arXiv:2001.03564 [hep-ph]].
%40 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Grover:1997fa}
\bibitem{Grover:1997fa}
L.~K.~Grover,
%``Quantum mechanics helps in searching for a needle in a haystack,''
Phys. Rev. Lett. \textbf{79} (1997), 325-328
doi:10.1103/PhysRevLett.79.325
[arXiv:quant-ph/9706033 [quant-ph]].
%427 citations counted in INSPIRE as of 22 Nov 2022

==> latexmkrc <==
###################################
#   Configuration script for build latex

#   The next lines are the original ones from source
#
#$pdf_previewer='zathura';
#$pdflatex='xelatex -synctex=1 %0 %S'
#@generated_exts=(@generated_exts, 'synctex.gz');

#   Compilation with Xelatex
$latex = 'latex --enable-write18 %O %S';
#$pdflatex='pdflatex -synctex=1 %0 %S';
#$pdf_mode=1;
$pdf_mode=5;
$dvi_mode=$postscript_mode=0;
#$dvipdf = "dvipdfm %O -o %D %S";


#   axodraw automation
add_cus_dep( "ax1", "ax2", 0, "axohelp");
sub axohelp {return system "axohelp \"$_[0]\"";}
$clean_ext .=" %R.ax1 %R.ax2;"

==> main-references.tex <==
%\cite{Catani:2008xa}
\bibitem{Catani:2008xa}
S.~Catani, T.~Gleisberg, F.~Krauss, G.~Rodrigo and J.~C.~Winter,
%``From loops to trees by-passing Feynman's theorem,''
JHEP \textbf{09} (2008), 065
doi:10.1088/1126-6708/2008/09/065
[arXiv:0804.3170 [hep-ph]].
%150 citations counted in INSPIRE as of 18 Nov 2022

%\cite{Tomboulis:2017rvd}
\bibitem{Tomboulis:2017rvd}
E.~T.~Tomboulis,
%``Causality and Unitarity via the Tree-Loop Duality Relation,''
JHEP \textbf{05} (2017), 148
doi:10.1007/JHEP05(2017)148
[arXiv:1701.07052 [hep-th]].
%37 citations counted in INSPIRE as of 18 Nov 2022

%\cite{deJesusAguilera-Verdugo:2021mvg}
\bibitem{deJesusAguilera-Verdugo:2021mvg}
J.~de Jes\'us Aguilera-Verdugo, F.~Driencourt-Mangin, R.~J.~Hern\'andez-Pinto, J.~Plenter, R.~M.~Prisco, N.~S.~Ram\'\i{}rez-Uribe, A.~E.~Renter\'\i{}a-Olivo, G.~Rodrigo, G.~Sborlini and W.~J.~Torres Bobadilla, \textit{et al.}
%``A Stroll through the Loop-Tree Duality,''
Symmetry \textbf{13} (2021) no.6, 1029
doi:10.3390/sym13061029
[arXiv:2104.14621 [hep-ph]].
%16 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Ramirez-Uribe:2021ubp}
\bibitem{Ramirez-Uribe:2021ubp}
S.~Ram\'\i{}rez-Uribe, A.~E.~Renter\'\i{}a-Olivo, G.~Rodrigo, G.~F.~R.~Sborlini and L.~Vale Silva,
%``Quantum algorithm for Feynman loop integrals,''
JHEP \textbf{05} (2022), 100
doi:10.1007/JHEP05(2022)100
[arXiv:2105.08703 [hep-ph]].
%19 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Clemente:2022nll}
\bibitem{Clemente:2022nll}
G.~Clemente, A.~Crippa, K.~Jansen, S.~Ram\'\i{}rez-Uribe, A.~E.~Renter\'\i{}a-Olivo, G.~Rodrigo, G.~F.~R.~Sborlini and L.~Vale Silva,
%``Variational quantum eigensolver for causal loop Feynman diagrams and acyclic directed graphs,''
[arXiv:2210.13240 [hep-ph]].
%1 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Aguilera-Verdugo:2020set}
\bibitem{Aguilera-Verdugo:2020set}
J.~J.~Aguilera-Verdugo, F.~Driencourt-Mangin, R.~J.~Hern\'andez-Pinto, J.~Plenter, S.~Ramirez-Uribe, A.~E.~Renteria Olivo, G.~Rodrigo, G.~F.~R.~Sborlini, W.~J.~Torres Bobadilla and S.~Tracz,
%``Open Loop Amplitudes and Causality to All Orders and Powers from the Loop-Tree Duality,''
Phys. Rev. Lett. \textbf{124} (2020) no.21, 211602
doi:10.1103/PhysRevLett.124.211602
[arXiv:2001.03564 [hep-ph]].
%40 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Grover:1997fa}
\bibitem{Grover:1997fa}
L.~K.~Grover,
%``Quantum mechanics helps in searching for a needle in a haystack,''
Phys. Rev. Lett. \textbf{79} (1997), 325-328
doi:10.1103/PhysRevLett.79.325
[arXiv:quant-ph/9706033 [quant-ph]].
%427 citations counted in INSPIRE as of 22 Nov 2022
